Hypervelocity Stars III. The Space Density and Ejection History of Main Sequence Stars from the Galactic Center

We report the discovery of 3 new unbound hypervelocity stars (HVSs), stars traveling with such extreme velocities that dynamical ejection from a massive black hole (MBH) is their only suggested origin. We also detect a population of possibly bound HVSs. The significant asymmetry we observe in the velocity distribution -- we find 26 stars with v_rf > 275 km/s and 1 star with v_rf < -275 km/s -- shows that the HVSs must be short-lived, probably 3 - 4 Msun main sequence stars. Any population of hypervelocity post-main sequence stars should contain stars falling back onto the Galaxy, contrary to the observations. The spatial distribution of HVSs also supports the main sequence interpretation: longer-lived 3 Msun HVSs fill our survey volume; shorter-lived 4 Msun HVSs are missing at faint magnitudes. We infer that there are 96 +- 10 HVSs of mass 3 - 4 Msun within R < 100 kpc, possibly enough HVSs to constrain ejection mechanisms and potential models. Depending on the mass function of HVSs, we predict that SEGUE may find up to 5 - 15 new HVSs. The travel times of our HVSs favor a continuous ejection process, although a ~120 Myr-old burst of HVSs is also allowed.

==> tab2.tex <==
 0:23:09.05 &  -0:33:42.0 & $16.277\pm0.020$ & $0.250\pm0.028$ & $-0.306\pm0.039$ & 1 & $ -13\pm31$ \\
 0:23:53.29 &  -1:04:46.4 & $18.304\pm0.016$ & $0.749\pm0.042$ & $-0.255\pm0.025$ & 0 & $  20\pm10$ \\
 0:43:50.55 &  -9:52:27.0 & $16.326\pm0.032$ & $0.832\pm0.038$ & $-0.358\pm0.038$ & 0 & $-117\pm11$ \\
 0:50:22.84 & -10:29:40.9 & $18.595\pm0.028$ & $0.629\pm0.045$ & $-0.264\pm0.033$ & 0 & $-110\pm10$ \\
 0:50:42.09 &  14:25:37.0 & $16.073\pm0.030$ & $1.199\pm0.039$ & $-0.291\pm0.036$ & 0 & $-214\pm11$ \\
 1:04:11.09 &   0:21:49.5 & $15.659\pm0.017$ & $0.752\pm0.022$ & $-0.326\pm0.024$ & 0 & $ -79\pm11$ \\
 1:04:32.24 &  15:41:50.3 & $15.531\pm0.022$ & $0.405\pm0.028$ & $-0.376\pm0.027$ & 0 & $ -29\pm11$ \\
 1:25:29.27 &   1:02:30.9 & $19.237\pm0.019$ & $0.808\pm0.052$ & $-0.263\pm0.033$ & 0 & $-139\pm10$ \\
 1:32:22.20 &   0:59:53.9 & $18.884\pm0.020$ & $0.452\pm0.039$ & $-0.326\pm0.027$ & 1 & $ -36\pm33$ \\
 1:33:56.07 &  -9:15:35.2 & $19.412\pm0.027$ & $0.473\pm0.061$ & $-0.331\pm0.034$ & 1 & $ -12\pm46$ \\
 1:34:41.75 &  -9:58:01.9 & $16.554\pm0.043$ & $0.102\pm0.046$ & $-0.351\pm0.045$ & 1 & $  17\pm40$ \\
 1:38:44.40 &  14:31:13.1 & $16.640\pm0.020$ & $0.789\pm0.026$ & $-0.317\pm0.024$ & 0 & $ -49\pm11$ \\
 1:48:07.02 &  -9:12:55.3 & $19.334\pm0.032$ & $0.396\pm0.055$ & $-0.349\pm0.038$ & 1 & $   5\pm29$ \\
 1:58:42.57 & -10:12:59.2 & $16.546\pm0.025$ & $0.971\pm0.030$ & $-0.292\pm0.029$ & 0 & $ 166\pm18$ \\
 2:05:07.73 &  -7:47:27.2 & $15.180\pm0.018$ & $1.077\pm0.024$ & $-0.286\pm0.035$ & 0 & $ -74\pm13$ \\
 2:16:21.23 &  -0:07:58.5 & $17.200\pm0.019$ & $0.388\pm0.024$ & $-0.349\pm0.022$ & 0 & $ 194\pm10$ \\
 2:19:09.35 &  -8:31:20.3 & $18.763\pm0.020$ & $0.475\pm0.035$ & $-0.309\pm0.025$ & 0 & $-136\pm10$ \\
 2:30:32.65 &  -8:14:39.5 & $15.870\pm0.015$ & $0.427\pm0.023$ & $-0.347\pm0.024$ & 0 & $-189\pm13$ \\
 2:40:15.08 &  -1:07:38.4 & $19.520\pm0.029$ & $0.319\pm0.049$ & $-0.369\pm0.036$ & 0 & $-131\pm10$ \\
 2:47:46.34 &   0:03:31.5 & $16.244\pm0.051$ & $0.164\pm0.053$ & $-0.456\pm0.056$ & 1 & $  -0\pm65$ \\
 2:54:50.00 &  -8:27:45.5 & $15.443\pm0.022$ & $1.080\pm0.024$ & $-0.310\pm0.044$ & 0 & $  91\pm14$ \\
 3:14:49.47 &  -7:48:22.0 & $19.799\pm0.034$ & $0.929\pm0.109$ & $-0.307\pm0.043$ & 0 & $ -86\pm11$ \\
 3:22:17.86 &  -5:59:55.2 & $16.813\pm0.018$ & $0.725\pm0.024$ & $-0.310\pm0.030$ & 0 & $ 139\pm12$ \\
 3:22:59.53 &  -8:01:56.8 & $19.453\pm0.031$ & $0.483\pm0.057$ & $-0.313\pm0.043$ & 1 & $   1\pm27$ \\
 3:23:02.87 &   0:05:59.6 & $17.436\pm0.023$ & $0.623\pm0.051$ & $-0.344\pm0.026$ & 1 & $  91\pm32$ \\
 3:26:19.45 &   0:18:17.3 & $17.420\pm0.016$ & $0.224\pm0.025$ & $-0.332\pm0.026$ & 1 & $  24\pm43$ \\
 7:47:15.71 &   8:54:32.6 & $16.438\pm0.009$ & $1.070\pm0.023$ & $-0.319\pm0.011$ & 0 & $  46\pm11$ \\
 7:47:59.70 &  42:12:42.8 & $19.226\pm0.015$ & $0.638\pm0.039$ & $-0.266\pm0.023$ & 1 & $  64\pm22$ \\
 7:49:31.81 &  13:30:58.8 & $15.427\pm0.016$ & $0.829\pm0.025$ & $-0.388\pm0.019$ & 0 & $   8\pm11$ \\
 7:50:41.72 &  19:11:54.5 & $19.170\pm0.024$ & $0.541\pm0.045$ & $-0.298\pm0.098$ & 1 & $   4\pm22$ \\
 7:51:25.11 &  12:02:34.6 & $16.480\pm0.012$ & $0.496\pm0.021$ & $-0.321\pm0.018$ & 0 & $ 296\pm11$ \\
 8:01:02.94 &  52:14:42.1 & $17.314\pm0.014$ & $0.518\pm0.024$ & $-0.360\pm0.027$ & 0 & $  -8\pm10$ \\
 8:01:33.59 &  33:05:00.2 & $17.273\pm0.016$ & $0.561\pm0.028$ & $-0.349\pm0.035$ & 0 & $  22\pm10$ \\
 8:11:33.56 &   2:25:56.8 & $18.685\pm0.013$ & $0.581\pm0.033$ & $-0.326\pm0.025$ & 0 & $ -42\pm12$ \\
 8:13:13.41 &  16:04:32.5 & $18.016\pm0.022$ & $0.885\pm0.033$ & $-0.327\pm0.028$ & 0 & $ 123\pm10$ \\
 8:20:17.56 &  57:54:15.7 & $18.474\pm0.043$ & $0.293\pm0.050$ & $-0.379\pm0.051$ & 1 & $  47\pm33$ \\
 8:22:57.56 &  18:44:00.3 & $16.332\pm0.014$ & $0.122\pm0.023$ & $-0.336\pm0.020$ & 1 & $  15\pm30$ \\
 8:27:59.49 &  49:26:52.0 & $19.509\pm0.043$ & $0.480\pm0.069$ & $-0.345\pm0.067$ & 1 & $ -53\pm26$ \\
 8:28:30.33 &  16:57:46.5 & $16.229\pm0.018$ & $0.309\pm0.022$ & $-0.359\pm0.025$ & 0 & $ 285\pm11$ \\
 8:31:32.75 &  13:22:43.9 & $15.906\pm0.017$ & $0.240\pm0.023$ & $-0.375\pm0.021$ & 1 & $  -3\pm32$ \\
 8:32:27.81 &  16:49:39.4 & $17.799\pm0.019$ & $0.728\pm0.031$ & $-0.289\pm0.028$ & 0 & $ -16\pm10$ \\
 8:39:01.51 &  16:11:48.0 & $16.465\pm0.023$ & $0.225\pm0.031$ & $-0.350\pm0.027$ & 0 & $ 199\pm12$ \\
 8:39:19.41 &  18:59:42.9 & $18.124\pm0.018$ & $0.623\pm0.035$ & $-0.306\pm0.027$ & 0 & $ 181\pm10$ \\
 8:48:21.44 &  16:42:34.0 & $19.281\pm0.021$ & $0.502\pm0.044$ & $-0.313\pm0.034$ & 1 & $  78\pm33$ \\
 8:49:01.75 &  15:18:34.5 & $15.575\pm0.024$ & $0.996\pm0.031$ & $-0.348\pm0.034$ & 0 & $   6\pm11$ \\
 8:53:53.51 &  22:16:29.0 & $16.551\pm0.013$ & $0.203\pm0.022$ & $-0.340\pm0.020$ & 1 & $  10\pm22$ \\
 8:55:30.66 &  19:04:37.5 & $16.318\pm0.016$ & $0.282\pm0.021$ & $-0.334\pm0.021$ & 1 & $ -56\pm34$ \\
 8:57:14.24 &  23:51:32.1 & $19.265\pm0.019$ & $0.388\pm0.040$ & $-0.355\pm0.068$ & 1 & $ 114\pm99$ \\
 9:04:44.56 &  20:02:21.3 & $16.577\pm0.022$ & $0.744\pm0.028$ & $-0.355\pm0.025$ & 0 & $ 251\pm10$ \\
 9:05:34.06 &   4:53:37.8 & $18.961\pm0.023$ & $0.841\pm0.050$ & $-0.277\pm0.032$ & 0 & $  16\pm11$ \\
 9:05:53.07 &  22:03:23.3 & $15.869\pm0.015$ & $0.874\pm0.026$ & $-0.301\pm0.019$ & 0 & $   5\pm11$ \\
 9:08:02.37 &  23:20:53.9 & $18.537\pm0.023$ & $0.341\pm0.033$ & $-0.365\pm0.030$ & 0 & $ -42\pm10$ \\
 9:11:24.00 &  16:54:11.7 & $15.913\pm0.016$ & $0.156\pm0.025$ & $-0.356\pm0.021$ & 1 & $  28\pm40$ \\
 9:16:33.43 &   2:58:53.0 & $17.606\pm0.018$ & $0.980\pm0.030$ & $-0.270\pm0.025$ & 0 & $  95\pm12$ \\
 9:19:58.62 &  20:40:21.2 & $17.119\pm0.017$ & $0.164\pm0.026$ & $-0.338\pm0.037$ & 1 & $ 118\pm44$ \\
 9:26:24.42 &  16:24:18.2 & $16.923\pm0.012$ & $1.340\pm0.022$ & $-0.299\pm0.026$ & 0 & $ -42\pm13$ \\
 9:26:43.75 &  20:59:59.8 & $18.160\pm0.016$ & $1.061\pm0.036$ & $-0.282\pm0.021$ & 0 & $ -35\pm10$ \\
 9:30:48.97 &  16:17:11.5 & $16.879\pm0.020$ & $0.598\pm0.030$ & $-0.371\pm0.030$ & 0 & $  24\pm11$ \\
 9:37:10.28 &  24:20:36.8 & $17.228\pm0.038$ & $1.160\pm0.045$ & $-0.289\pm0.042$ & 0 & $  42\pm11$ \\
 9:42:14.04 &  20:03:22.1 & $18.045\pm0.016$ & $0.780\pm0.025$ & $-0.315\pm0.022$ & 0 & $ 512\pm10$ \\
 9:51:28.61 &  24:30:36.1 & $18.565\pm0.016$ & $0.886\pm0.033$ & $-0.290\pm0.025$ & 0 & $  55\pm10$ \\
 9:52:10.08 &  23:01:23.9 & $18.446\pm0.022$ & $1.098\pm0.036$ & $-0.285\pm0.027$ & 0 & $  32\pm10$ \\
 9:59:29.85 &  22:09:21.9 & $16.323\pm0.022$ & $0.222\pm0.027$ & $-0.362\pm0.028$ & 0 & $  99\pm11$ \\
 9:59:51.18 &   5:21:24.5 & $19.346\pm0.022$ & $0.833\pm0.054$ & $-0.262\pm0.030$ & 0 & $ 294\pm11$ \\
10:03:56.09 &  19:39:41.3 & $17.233\pm0.017$ & $0.816\pm0.028$ & $-0.298\pm0.028$ & 0 & $ 212\pm10$ \\
10:04:17.95 &  22:40:44.4 & $18.458\pm0.021$ & $0.982\pm0.037$ & $-0.319\pm0.028$ & 0 & $ 216\pm10$ \\
10:07:38.31 &  18:32:20.3 & $18.069\pm0.024$ & $0.745\pm0.033$ & $-0.299\pm0.028$ & 0 & $ -24\pm10$ \\
10:08:35.25 &  23:52:45.6 & $17.450\pm0.019$ & $0.783\pm0.030$ & $-0.300\pm0.024$ & 0 & $ 140\pm10$ \\
10:13:37.64 &  27:20:45.6 & $18.137\pm0.028$ & $0.699\pm0.037$ & $-0.275\pm0.032$ & 0 & $ -62\pm11$ \\
10:16:13.33 &  24:00:08.4 & $16.751\pm0.019$ & $0.531\pm0.024$ & $-0.364\pm0.022$ & 0 & $ 209\pm15$ \\
10:18:27.84 &  20:57:50.4 & $19.136\pm0.030$ & $0.684\pm0.048$ & $-0.298\pm0.035$ & 0 & $ 205\pm11$ \\
10:21:37.08 &  -0:52:34.8 & $18.842\pm0.024$ & $0.784\pm0.038$ & $-0.263\pm0.028$ & 0 & $ 632\pm11$ \\
10:23:01.12 &   6:08:21.3 & $19.171\pm0.017$ & $0.886\pm0.047$ & $-0.261\pm0.026$ & 0 & $  48\pm10$ \\
10:23:20.67 &   7:59:34.1 & $16.704\pm0.034$ & $0.133\pm0.037$ & $-0.456\pm0.042$ & 0 & $ 141\pm14$ \\
10:24:15.42 &  29:31:45.2 & $19.503\pm0.020$ & $0.884\pm0.062$ & $-0.275\pm0.031$ & 0 & $  94\pm10$ \\
10:26:52.71 &  62:44:06.1 & $16.352\pm0.085$ & $0.322\pm0.090$ & $-0.332\pm0.273$ & 1 & $ -61\pm59$ \\
10:27:12.84 &  20:44:22.6 & $17.536\pm0.020$ & $0.597\pm0.028$ & $-0.321\pm0.025$ & 0 & $ -95\pm10$ \\
10:28:08.34 &  23:21:40.1 & $15.081\pm0.023$ & $0.964\pm0.033$ & $-0.299\pm0.033$ & 0 & $ 343\pm11$ \\
10:29:54.80 &  22:46:11.7 & $19.461\pm0.020$ & $0.615\pm0.043$ & $-0.280\pm0.030$ & 0 & $ 176\pm10$ \\
10:30:43.94 &  24:41:43.6 & $17.570\pm0.023$ & $0.828\pm0.029$ & $-0.264\pm0.028$ & 0 & $ -13\pm11$ \\
10:34:02.07 &  21:30:09.0 & $15.617\pm0.018$ & $0.791\pm0.025$ & $-0.300\pm0.024$ & 0 & $  33\pm10$ \\
10:40:42.21 &  26:27:48.8 & $16.634\pm0.013$ & $0.123\pm0.027$ & $-0.321\pm0.021$ & 1 & $  99\pm24$ \\
10:41:21.49 &  21:03:33.9 & $18.982\pm0.025$ & $0.664\pm0.039$ & $-0.276\pm0.033$ & 0 & $ -63\pm10$ \\
10:41:33.64 &  19:03:11.8 & $17.892\pm0.029$ & $0.613\pm0.036$ & $-0.291\pm0.034$ & 0 & $  86\pm10$ \\
10:43:15.84 &  19:28:42.4 & $15.467\pm0.014$ & $0.683\pm0.034$ & $-0.297\pm0.017$ & 0 & $ 153\pm10$ \\
10:44:47.09 &  27:08:43.6 & $15.340\pm0.027$ & $1.002\pm0.031$ & $-0.295\pm0.031$ & 0 & $-129\pm11$ \\
10:47:11.63 &  21:34:08.3 & $16.449\pm0.022$ & $0.323\pm0.027$ & $-0.393\pm0.026$ & 0 & $ 266\pm12$ \\
10:51:34.99 &  54:27:52.2 & $19.387\pm0.029$ & $0.949\pm0.071$ & $-0.280\pm0.038$ & 0 & $-107\pm14$ \\
10:51:40.33 &  18:45:46.1 & $17.227\pm0.017$ & $0.892\pm0.029$ & $-0.261\pm0.022$ & 0 & $ 282\pm11$ \\
10:52:08.16 &   0:34:44.5 & $19.017\pm0.021$ & $0.642\pm0.043$ & $-0.264\pm0.031$ & 0 & $ 142\pm11$ \\
10:54:10.34 &  22:03:13.4 & $16.732\pm0.031$ & $0.340\pm0.039$ & $-0.313\pm0.041$ & 1 & $ -40\pm42$ \\
10:55:14.67 &  25:06:02.3 & $17.105\pm0.023$ & $0.936\pm0.030$ & $-0.293\pm0.033$ & 0 & $ 198\pm15$ \\
10:58:38.44 &  22:49:40.2 & $16.756\pm0.021$ & $0.108\pm0.024$ & $-0.412\pm0.030$ & 1 & $  83\pm41$ \\
11:02:06.36 &  26:22:01.9 & $19.165\pm0.019$ & $1.007\pm0.050$ & $-0.285\pm0.028$ & 0 & $ -49\pm10$ \\
11:02:41.99 &  25:18:40.9 & $15.247\pm0.019$ & $0.805\pm0.022$ & $-0.286\pm0.022$ & 0 & $ 139\pm10$ \\
11:03:22.48 &  18:59:15.2 & $16.274\pm0.017$ & $1.369\pm0.023$ & $-0.284\pm0.021$ & 0 & $ 138\pm13$ \\
11:04:43.31 &  27:59:45.1 & $16.569\pm0.019$ & $0.960\pm0.031$ & $-0.294\pm0.025$ & 0 & $  91\pm11$ \\
11:07:21.15 &  18:46:02.8 & $17.336\pm0.017$ & $0.885\pm0.024$ & $-0.323\pm0.023$ & 0 & $ 189\pm10$ \\
11:09:33.38 &  23:27:52.8 & $18.257\pm0.016$ & $1.073\pm0.035$ & $-0.301\pm0.036$ & 0 & $  40\pm11$ \\
11:10:25.57 &  17:56:30.4 & $19.405\pm0.022$ & $0.539\pm0.056$ & $-0.297\pm0.033$ & 1 & $  17\pm19$ \\
11:10:48.19 &  23:18:21.1 & $18.035\pm0.021$ & $0.627\pm0.030$ & $-0.296\pm0.033$ & 0 & $ 104\pm10$ \\
11:12:52.43 &  19:57:23.9 & $18.729\pm0.022$ & $0.798\pm0.039$ & $-0.265\pm0.027$ & 0 & $ -22\pm10$ \\
11:13:03.60 &  27:12:59.1 & $18.588\pm0.017$ & $0.836\pm0.045$ & $-0.288\pm0.029$ & 0 & $  94\pm11$ \\
11:13:23.71 &  16:28:56.2 & $18.429\pm0.015$ & $0.618\pm0.031$ & $-0.312\pm0.023$ & 0 & $ -20\pm10$ \\
11:16:57.26 &   1:31:51.2 & $19.338\pm0.026$ & $0.834\pm0.050$ & $-0.259\pm0.031$ & 0 & $ 180\pm14$ \\
11:17:55.64 &  20:45:34.5 & $18.722\pm0.028$ & $0.487\pm0.037$ & $-0.373\pm0.037$ & 0 & $ -30\pm10$ \\
11:20:35.48 &  18:41:53.2 & $17.674\pm0.021$ & $0.662\pm0.032$ & $-0.284\pm0.028$ & 0 & $-137\pm10$ \\
11:20:59.69 &  17:35:19.7 & $17.070\pm0.019$ & $0.185\pm0.034$ & $-0.383\pm0.023$ & 1 & $ -38\pm28$ \\
11:22:24.92 &  17:58:09.2 & $16.206\pm0.019$ & $0.732\pm0.042$ & $-0.337\pm0.029$ & 0 & $ 165\pm10$ \\
11:22:36.96 &  13:47:36.9 & $19.023\pm0.031$ & $0.877\pm0.048$ & $-0.324\pm0.037$ & 0 & $  45\pm10$ \\
11:22:44.78 &   6:23:03.5 & $19.701\pm0.030$ & $0.704\pm0.064$ & $-0.366\pm0.039$ & 0 & $ 168\pm10$ \\
11:26:01.48 &  22:29:04.8 & $18.232\pm0.019$ & $1.017\pm0.034$ & $-0.295\pm0.030$ & 0 & $ -28\pm12$ \\
11:26:06.25 &  -0:06:45.3 & $18.476\pm0.021$ & $0.749\pm0.030$ & $-0.260\pm0.026$ & 0 & $ 170\pm10$ \\
11:26:31.38 &  11:14:06.2 & $19.194\pm0.030$ & $1.111\pm0.078$ & $-0.288\pm0.043$ & 0 & $ 103\pm10$ \\
11:27:01.79 &  21:55:49.9 & $16.894\pm0.019$ & $0.194\pm0.034$ & $-0.388\pm0.022$ & 1 & $ -12\pm51$ \\
11:32:40.19 &  15:58:45.4 & $18.874\pm0.021$ & $0.375\pm0.041$ & $-0.377\pm0.026$ & 0 & $ 110\pm10$ \\
11:33:41.09 &  -1:21:14.3 & $19.240\pm0.020$ & $0.815\pm0.054$ & $-0.348\pm0.031$ & 0 & $ 463\pm11$ \\
11:35:01.18 &  17:04:44.0 & $18.779\pm0.023$ & $0.634\pm0.038$ & $-0.310\pm0.030$ & 0 & $ -39\pm10$ \\
11:35:10.19 &  30:14:29.5 & $17.329\pm0.023$ & $1.086\pm0.036$ & $-0.309\pm0.030$ & 0 & $ 168\pm10$ \\
11:35:21.02 &  28:46:05.1 & $16.462\pm0.017$ & $1.125\pm0.022$ & $-0.283\pm0.021$ & 0 & $  58\pm10$ \\
11:36:22.85 &  18:30:49.9 & $16.908\pm0.028$ & $0.383\pm0.035$ & $-0.335\pm0.034$ & 0 & $-177\pm13$ \\
11:37:30.16 &  27:25:27.9 & $17.850\pm0.025$ & $0.961\pm0.037$ & $-0.295\pm0.033$ & 0 & $  -6\pm10$ \\
11:37:36.32 &  26:21:53.5 & $17.506\pm0.020$ & $1.123\pm0.030$ & $-0.292\pm0.023$ & 0 & $  36\pm10$ \\
11:37:48.43 &  26:32:15.7 & $17.581\pm0.025$ & $0.929\pm0.036$ & $-0.325\pm0.030$ & 0 & $  90\pm10$ \\
11:38:11.39 &  26:44:41.7 & $15.373\pm0.018$ & $0.207\pm0.038$ & $-0.326\pm0.025$ & 1 & $  47\pm30$ \\
11:39:26.59 &   6:41:25.9 & $19.130\pm0.022$ & $0.812\pm0.051$ & $-0.318\pm0.028$ & 0 & $ -35\pm12$ \\
11:39:47.08 &  17:43:58.1 & $18.378\pm0.017$ & $0.899\pm0.038$ & $-0.280\pm0.026$ & 0 & $ -25\pm10$ \\
11:40:32.41 &  25:57:21.4 & $16.481\pm0.019$ & $0.730\pm0.031$ & $-0.342\pm0.026$ & 0 & $  13\pm16$ \\
11:41:32.71 &  21:03:53.7 & $16.218\pm0.016$ & $1.029\pm0.024$ & $-0.324\pm0.032$ & 0 & $ 163\pm14$ \\
11:43:35.80 &  19:14:24.2 & $17.645\pm0.025$ & $0.979\pm0.039$ & $-0.313\pm0.033$ & 0 & $-151\pm11$ \\
11:44:18.51 &  27:48:28.7 & $17.651\pm0.018$ & $0.875\pm0.036$ & $-0.282\pm0.024$ & 0 & $  56\pm10$ \\
11:44:39.13 &  29:14:39.2 & $18.490\pm0.015$ & $0.735\pm0.036$ & $-0.288\pm0.027$ & 0 & $-105\pm12$ \\
11:45:08.75 &   9:34:53.3 & $18.499\pm0.024$ & $1.069\pm0.040$ & $-0.307\pm0.027$ & 0 & $  38\pm11$ \\
11:47:25.75 &  17:15:50.7 & $19.007\pm0.024$ & $0.758\pm0.053$ & $-0.316\pm0.029$ & 0 & $  -4\pm10$ \\
11:48:16.52 &  18:00:58.7 & $18.842\pm0.021$ & $0.790\pm0.043$ & $-0.329\pm0.027$ & 0 & $ -19\pm10$ \\
11:48:56.92 &  25:18:14.5 & $18.097\pm0.033$ & $1.033\pm0.045$ & $-0.282\pm0.040$ & 0 & $ -60\pm10$ \\
11:51:27.18 &   8:50:30.3 & $18.774\pm0.031$ & $0.452\pm0.040$ & $-0.342\pm0.038$ & 0 & $  98\pm10$ \\
11:52:18.24 &  27:48:25.9 & $18.648\pm0.050$ & $0.416\pm0.056$ & $-0.340\pm0.055$ & 1 & $  48\pm33$ \\
11:53:15.09 &  17:06:58.2 & $15.197\pm0.020$ & $0.917\pm0.030$ & $-0.295\pm0.026$ & 0 & $ 158\pm11$ \\
11:53:35.96 &  20:04:14.1 & $18.537\pm0.034$ & $1.057\pm0.050$ & $-0.299\pm0.038$ & 0 & $ -67\pm10$ \\
11:53:45.61 &   7:21:31.4 & $18.854\pm0.029$ & $0.914\pm0.048$ & $-0.297\pm0.035$ & 0 & $  49\pm11$ \\
11:55:20.95 &  22:47:54.6 & $19.417\pm0.025$ & $0.409\pm0.045$ & $-0.362\pm0.033$ & 1 & $ -55\pm35$ \\
12:00:17.59 &   1:50:17.8 & $18.733\pm0.021$ & $0.762\pm0.047$ & $-0.334\pm0.027$ & 0 & $ 197\pm10$ \\
12:00:28.38 &  19:56:21.9 & $18.835\pm0.021$ & $0.550\pm0.047$ & $-0.280\pm0.025$ & 0 & $ -62\pm10$ \\
12:01:04.31 &  22:52:49.2 & $15.850\pm0.028$ & $0.838\pm0.036$ & $-0.339\pm0.055$ & 0 & $ 276\pm14$ \\
12:03:11.26 &   4:54:19.6 & $18.599\pm0.025$ & $0.641\pm0.039$ & $-0.348\pm0.030$ & 0 & $ 333\pm10$ \\
12:03:37.86 &  18:02:50.3 & $19.295\pm0.024$ & $0.826\pm0.058$ & $-0.290\pm0.033$ & 0 & $ 478\pm10$ \\
12:03:58.08 &  12:03:12.3 & $19.530\pm0.015$ & $0.824\pm0.063$ & $-0.270\pm0.029$ & 0 & $  10\pm11$ \\
12:04:34.73 &   4:26:18.5 & $18.514\pm0.022$ & $1.050\pm0.039$ & $-0.294\pm0.025$ & 0 & $ 103\pm14$ \\
12:05:08.16 &  24:03:32.0 & $15.304\pm0.034$ & $1.005\pm0.037$ & $-0.309\pm0.039$ & 0 & $  92\pm10$ \\
12:06:20.42 &  -3:16:55.8 & $17.695\pm0.033$ & $1.004\pm0.053$ & $-0.310\pm0.047$ & 0 & $  89\pm11$ \\
12:07:32.99 &  17:36:21.0 & $19.487\pm0.025$ & $0.998\pm0.091$ & $-0.295\pm0.039$ & 0 & $ -45\pm11$ \\
12:09:24.23 &  16:30:24.6 & $16.833\pm0.031$ & $0.161\pm0.038$ & $-0.326\pm0.040$ & 1 & $-225\pm64$ \\
12:11:58.87 &  17:51:44.3 & $15.179\pm0.022$ & $0.433\pm0.024$ & $-0.334\pm0.027$ & 0 & $  67\pm12$ \\
12:12:28.70 &  18:00:40.2 & $17.477\pm0.020$ & $0.780\pm0.042$ & $-0.302\pm0.034$ & 0 & $ 200\pm10$ \\
12:13:31.15 &  18:54:14.1 & $19.474\pm0.026$ & $0.856\pm0.063$ & $-0.274\pm0.033$ & 0 & $  20\pm11$ \\
12:14:33.20 &  22:16:17.4 & $17.767\pm0.029$ & $0.936\pm0.036$ & $-0.299\pm0.051$ & 0 & $-143\pm10$ \\
12:14:36.26 &  18:32:36.7 & $17.047\pm0.016$ & $0.962\pm0.026$ & $-0.289\pm0.023$ & 0 & $ -81\pm12$ \\
12:14:42.20 &  14:21:48.7 & $18.955\pm0.022$ & $0.545\pm0.042$ & $-0.349\pm0.032$ & 0 & $ -49\pm10$ \\
12:15:05.95 &  12:08:37.0 & $19.016\pm0.021$ & $0.869\pm0.052$ & $-0.287\pm0.030$ & 0 & $   9\pm10$ \\
12:15:24.90 &  30:53:00.8 & $18.536\pm0.022$ & $0.565\pm0.047$ & $-0.345\pm0.031$ & 0 & $ 174\pm10$ \\
12:16:06.29 &  19:19:56.8 & $17.650\pm0.027$ & $1.043\pm0.036$ & $-0.289\pm0.034$ & 0 & $  86\pm10$ \\
12:16:19.96 &  -0:02:05.0 & $19.376\pm0.020$ & $0.630\pm0.042$ & $-0.280\pm0.028$ & 1 & $  20\pm24$ \\
12:16:21.34 &  16:48:25.3 & $17.048\pm0.018$ & $0.865\pm0.027$ & $-0.336\pm0.025$ & 0 & $ 246\pm11$ \\
12:16:25.83 &  -1:48:04.6 & $18.551\pm0.017$ & $0.585\pm0.033$ & $-0.368\pm0.025$ & 0 & $  99\pm10$ \\
12:18:00.45 &  29:51:38.3 & $15.995\pm0.029$ & $0.853\pm0.034$ & $-0.345\pm0.035$ & 0 & $-173\pm10$ \\
12:18:23.29 &  23:16:11.9 & $19.282\pm0.025$ & $0.587\pm0.041$ & $-0.349\pm0.031$ & 0 & $ -72\pm10$ \\
12:20:54.02 &  22:42:12.3 & $15.986\pm0.021$ & $0.780\pm0.027$ & $-0.375\pm0.034$ & 0 & $ 163\pm12$ \\
12:21:18.30 &  -0:16:52.0 & $17.750\pm0.018$ & $0.584\pm0.032$ & $-0.319\pm0.024$ & 0 & $ 160\pm11$ \\
12:21:44.00 &  29:53:08.8 & $18.354\pm0.029$ & $0.944\pm0.042$ & $-0.330\pm0.034$ & 0 & $ -34\pm10$ \\
12:21:53.43 &  28:20:06.2 & $17.240\pm0.018$ & $0.740\pm0.025$ & $-0.307\pm0.024$ & 0 & $ -30\pm10$ \\
12:22:00.88 &  12:41:30.8 & $19.642\pm0.032$ & $1.039\pm0.097$ & $-0.288\pm0.041$ & 0 & $   0\pm12$ \\
12:23:10.92 &  31:04:30.3 & $19.225\pm0.053$ & $1.121\pm0.091$ & $-0.289\pm0.057$ & 0 & $ -59\pm11$ \\
12:23:33.92 &  22:08:20.9 & $16.753\pm0.026$ & $0.205\pm0.048$ & $-0.309\pm0.034$ & 1 & $  -2\pm23$ \\
12:23:52.64 &   3:33:47.7 & $17.519\pm0.021$ & $0.841\pm0.037$ & $-0.319\pm0.026$ & 0 & $  46\pm10$ \\
12:24:13.60 &  21:51:53.8 & $18.249\pm0.033$ & $1.085\pm0.046$ & $-0.342\pm0.041$ & 0 & $  92\pm11$ \\
12:25:10.92 &   2:03:18.2 & $18.866\pm0.028$ & $0.820\pm0.053$ & $-0.343\pm0.033$ & 0 & $ 130\pm10$ \\
12:25:30.95 &  23:04:46.0 & $17.284\pm0.028$ & $1.137\pm0.068$ & $-0.301\pm0.038$ & 0 & $ -64\pm10$ \\
12:26:02.45 &   2:54:07.7 & $18.942\pm0.018$ & $0.936\pm0.048$ & $-0.294\pm0.028$ & 0 & $ -18\pm11$ \\
12:27:12.54 &  21:51:49.2 & $15.514\pm0.022$ & $0.784\pm0.027$ & $-0.307\pm0.029$ & 0 & $ 117\pm11$ \\
12:27:15.24 &  23:39:37.3 & $18.470\pm0.018$ & $0.891\pm0.036$ & $-0.274\pm0.025$ & 0 & $ -51\pm10$ \\
12:27:42.06 &  11:12:02.3 & $19.615\pm0.031$ & $0.700\pm0.080$ & $-0.278\pm0.044$ & 0 & $ -46\pm12$ \\
12:28:26.73 &  26:50:55.7 & $18.968\pm0.018$ & $0.564\pm0.051$ & $-0.291\pm0.029$ & 0 & $-176\pm11$ \\
12:28:28.55 &  28:17:06.9 & $17.035\pm0.018$ & $1.044\pm0.031$ & $-0.286\pm0.024$ & 0 & $ -50\pm15$ \\
12:28:33.90 &  -1:23:11.7 & $17.424\pm0.022$ & $0.754\pm0.030$ & $-0.327\pm0.026$ & 0 & $ -19\pm10$ \\
12:29:07.28 &  23:24:34.0 & $18.079\pm0.022$ & $0.986\pm0.066$ & $-0.302\pm0.035$ & 0 & $-128\pm10$ \\
12:32:01.41 &  27:30:24.4 & $17.707\pm0.034$ & $0.539\pm0.041$ & $-0.295\pm0.039$ & 0 & $  14\pm10$ \\
12:33:56.28 &  23:08:19.1 & $15.756\pm0.032$ & $1.042\pm0.034$ & $-0.291\pm0.034$ & 0 & $  11\pm10$ \\
12:33:58.32 &  16:23:11.3 & $17.258\pm0.029$ & $1.017\pm0.042$ & $-0.294\pm0.033$ & 0 & $-118\pm10$ \\
12:34:03.85 &  13:09:10.0 & $19.487\pm0.026$ & $0.645\pm0.053$ & $-0.337\pm0.035$ & 0 & $ -32\pm14$ \\
12:35:07.34 &   0:20:05.9 & $19.061\pm0.017$ & $1.017\pm0.046$ & $-0.306\pm0.023$ & 0 & $ -29\pm11$ \\
12:36:38.17 &  22:05:06.3 & $18.300\pm0.033$ & $1.089\pm0.051$ & $-0.288\pm0.038$ & 0 & $  68\pm11$ \\
12:36:40.08 &  22:09:17.7 & $15.976\pm0.033$ & $0.468\pm0.044$ & $-0.348\pm0.038$ & 0 & $ 101\pm12$ \\
12:38:00.10 &  19:46:31.4 & $17.265\pm0.019$ & $0.486\pm0.025$ & $-0.365\pm0.025$ & 0 & $-185\pm11$ \\
12:38:06.07 &  17:14:39.2 & $15.693\pm0.025$ & $1.225\pm0.030$ & $-0.297\pm0.030$ & 0 & $ -70\pm11$ \\
12:38:29.52 &  16:43:34.8 & $17.943\pm0.021$ & $0.771\pm0.034$ & $-0.272\pm0.029$ & 0 & $  -2\pm12$ \\
12:38:42.79 &  24:05:37.5 & $19.148\pm0.022$ & $0.810\pm0.056$ & $-0.259\pm0.028$ & 0 & $ -78\pm11$ \\
12:39:10.99 &  12:52:56.7 & $19.507\pm0.025$ & $0.577\pm0.052$ & $-0.329\pm0.034$ & 0 & $   0\pm11$ \\
12:39:43.22 &   5:39:07.0 & $19.190\pm0.021$ & $0.418\pm0.038$ & $-0.363\pm0.030$ & 1 & $   2\pm51$ \\
12:39:49.47 &   9:02:10.5 & $19.224\pm0.020$ & $1.037\pm0.071$ & $-0.303\pm0.036$ & 0 & $   7\pm11$ \\
12:40:45.61 &  17:39:11.5 & $18.086\pm0.015$ & $0.879\pm0.028$ & $-0.304\pm0.020$ & 0 & $ -32\pm12$ \\
12:40:48.61 &  -3:37:08.4 & $18.621\pm0.018$ & $0.994\pm0.037$ & $-0.286\pm0.024$ & 0 & $ -88\pm14$ \\
12:41:09.99 &  21:56:11.1 & $17.925\pm0.027$ & $1.112\pm0.035$ & $-0.281\pm0.030$ & 0 & $ 138\pm11$ \\
12:41:46.34 &  27:53:11.9 & $18.808\pm0.027$ & $0.959\pm0.047$ & $-0.327\pm0.035$ & 0 & $-141\pm11$ \\
12:42:19.70 &  27:27:56.0 & $16.246\pm0.019$ & $0.302\pm0.024$ & $-0.318\pm0.042$ & 1 & $  15\pm33$ \\
12:43:20.13 &   9:27:13.2 & $17.772\pm0.015$ & $0.826\pm0.032$ & $-0.326\pm0.023$ & 0 & $ -17\pm11$ \\
12:43:38.94 &  -2:09:51.9 & $18.826\pm0.020$ & $0.853\pm0.041$ & $-0.341\pm0.034$ & 0 & $ 325\pm11$ \\
12:43:50.94 &  28:42:35.9 & $15.246\pm0.013$ & $0.838\pm0.019$ & $-0.309\pm0.026$ & 0 & $ -85\pm10$ \\
12:46:04.75 &  29:54:39.1 & $18.074\pm0.018$ & $0.586\pm0.027$ & $-0.251\pm0.025$ & 1 & $ -12\pm16$ \\
12:46:11.50 &   2:17:15.2 & $18.060\pm0.013$ & $0.767\pm0.027$ & $-0.287\pm0.025$ & 0 & $ 124\pm10$ \\
12:47:37.48 &   4:04:09.2 & $19.277\pm0.021$ & $0.647\pm0.045$ & $-0.333\pm0.030$ & 0 & $  49\pm10$ \\
12:47:54.80 &   4:59:28.7 & $19.036\pm0.048$ & $0.544\pm0.069$ & $-0.305\pm0.053$ & 1 & $ -27\pm28$ \\
12:48:34.38 &   1:46:06.9 & $19.421\pm0.027$ & $0.989\pm0.077$ & $-0.332\pm0.037$ & 0 & $ 302\pm10$ \\
12:49:02.01 &  -3:22:37.0 & $18.631\pm0.023$ & $0.725\pm0.039$ & $-0.255\pm0.029$ & 0 & $ 154\pm10$ \\
12:49:31.87 &  -2:51:21.6 & $18.247\pm0.016$ & $0.823\pm0.034$ & $-0.262\pm0.024$ & 0 & $ -17\pm16$ \\
12:50:02.15 &   1:55:29.7 & $18.026\pm0.018$ & $0.934\pm0.033$ & $-0.302\pm0.023$ & 0 & $ 128\pm10$ \\
12:51:16.05 &  15:16:13.8 & $19.274\pm0.017$ & $0.356\pm0.039$ & $-0.370\pm0.028$ & 0 & $ 256\pm17$ \\
12:52:41.94 &  19:15:27.2 & $16.553\pm0.011$ & $0.122\pm0.017$ & $-0.341\pm0.016$ & 1 & $  39\pm29$ \\
12:53:46.52 &  22:37:40.6 & $16.787\pm0.087$ & $0.220\pm0.092$ & $-0.363\pm0.096$ & 1 & $ -41\pm26$ \\
12:54:05.94 &   2:01:16.3 & $17.539\pm0.021$ & $0.493\pm0.036$ & $-0.348\pm0.026$ & 0 & $ 248\pm10$ \\
12:55:53.39 &  15:25:55.1 & $19.506\pm0.017$ & $0.342\pm0.047$ & $-0.361\pm0.033$ & 1 & $ 100\pm65$ \\
12:59:18.51 &  10:16:43.9 & $18.829\pm0.025$ & $1.034\pm0.044$ & $-0.305\pm0.129$ & 0 & $  85\pm12$ \\
12:59:26.03 &  27:21:22.7 & $15.115\pm0.025$ & $0.114\pm0.031$ & $-0.455\pm0.031$ & 0 & $  16\pm10$ \\
12:59:32.56 &   7:55:29.3 & $17.467\pm0.015$ & $1.022\pm0.023$ & $-0.282\pm0.023$ & 0 & $ 142\pm11$ \\
13:00:22.10 &   9:07:34.2 & $19.456\pm0.020$ & $1.018\pm0.066$ & $-0.316\pm0.031$ & 0 & $ 164\pm21$ \\
13:02:30.67 &   5:32:37.2 & $18.876\pm0.017$ & $0.971\pm0.039$ & $-0.292\pm0.025$ & 0 & $ 128\pm13$ \\
13:03:23.70 &  25:10:07.6 & $16.151\pm0.011$ & $0.154\pm0.020$ & $-0.339\pm0.021$ & 1 & $ 103\pm36$ \\
13:03:27.64 &   5:47:07.1 & $18.111\pm0.017$ & $0.959\pm0.043$ & $-0.306\pm0.025$ & 0 & $ -84\pm11$ \\
13:06:55.88 &  31:58:38.9 & $15.979\pm0.028$ & $1.089\pm0.038$ & $-0.300\pm0.032$ & 0 & $ -13\pm12$ \\
13:10:24.97 &   4:57:17.3 & $17.214\pm0.018$ & $0.876\pm0.028$ & $-0.288\pm0.026$ & 0 & $ 199\pm11$ \\
13:11:04.74 &  32:38:21.1 & $16.041\pm0.023$ & $0.114\pm0.024$ & $-0.348\pm0.029$ & 1 & $  90\pm36$ \\
13:12:14.20 &  18:01:46.1 & $17.121\pm0.026$ & $1.006\pm0.036$ & $-0.287\pm0.032$ & 0 & $ -38\pm11$ \\
13:12:50.31 &  18:18:13.9 & $17.267\pm0.025$ & $0.900\pm0.035$ & $-0.277\pm0.029$ & 0 & $ -40\pm11$ \\
13:12:56.28 &  31:41:02.4 & $15.505\pm0.020$ & $0.950\pm0.026$ & $-0.287\pm0.023$ & 0 & $ -20\pm10$ \\
13:16:38.53 &  17:37:00.4 & $17.039\pm0.014$ & $1.031\pm0.024$ & $-0.314\pm0.021$ & 0 & $  24\pm11$ \\
13:22:38.27 &  24:29:57.3 & $16.914\pm0.020$ & $0.955\pm0.032$ & $-0.333\pm0.028$ & 0 & $-144\pm12$ \\
13:23:39.57 &  16:57:57.4 & $18.605\pm0.019$ & $0.607\pm0.036$ & $-0.281\pm0.022$ & 1 & $  63\pm21$ \\
13:24:36.40 &  20:38:17.1 & $15.429\pm0.017$ & $1.021\pm0.038$ & $-0.313\pm0.025$ & 0 & $  33\pm13$ \\
13:25:03.16 &   4:32:39.4 & $18.348\pm0.023$ & $0.484\pm0.031$ & $-0.342\pm0.030$ & 0 & $-155\pm11$ \\
13:25:52.40 &  20:35:24.8 & $15.441\pm0.047$ & $1.331\pm0.055$ & $-0.296\pm0.051$ & 0 & $ -90\pm21$ \\
13:28:07.49 &  20:51:51.1 & $17.491\pm0.023$ & $1.008\pm0.033$ & $-0.294\pm0.030$ & 0 & $-189\pm12$ \\
13:30:24.58 &  19:21:47.4 & $17.628\pm0.013$ & $0.589\pm0.028$ & $-0.273\pm0.027$ & 0 & $ -74\pm10$ \\
13:31:40.80 &   2:43:04.2 & $19.440\pm0.018$ & $0.889\pm0.058$ & $-0.313\pm0.028$ & 0 & $ 243\pm10$ \\
13:33:02.15 &  25:16:18.3 & $17.997\pm0.019$ & $0.521\pm0.029$ & $-0.320\pm0.022$ & 0 & $ -36\pm11$ \\
13:33:17.62 &   3:21:01.6 & $15.644\pm0.019$ & $0.144\pm0.026$ & $-0.367\pm0.024$ & 1 & $  84\pm34$ \\
13:33:40.28 &   2:48:45.8 & $17.090\pm0.021$ & $0.155\pm0.030$ & $-0.370\pm0.028$ & 1 & $ -32\pm44$ \\
13:34:33.90 &  -1:40:06.4 & $16.344\pm0.039$ & $0.189\pm0.044$ & $-0.395\pm0.046$ & 1 & $  29\pm42$ \\
13:34:41.32 &  25:56:46.2 & $16.633\pm0.018$ & $0.186\pm0.027$ & $-0.329\pm0.026$ & 1 & $  84\pm45$ \\
13:34:44.81 &  24:03:08.4 & $19.458\pm0.019$ & $0.843\pm0.053$ & $-0.259\pm0.027$ & 0 & $ 154\pm17$ \\
13:35:10.94 &   6:12:34.5 & $18.346\pm0.025$ & $0.524\pm0.033$ & $-0.338\pm0.029$ & 0 & $  18\pm10$ \\
13:35:19.90 &   6:40:09.3 & $15.711\pm0.018$ & $0.851\pm0.048$ & $-0.294\pm0.024$ & 0 & $ -13\pm11$ \\
13:35:42.59 &   2:13:57.5 & $19.477\pm0.023$ & $0.976\pm0.067$ & $-0.285\pm0.030$ & 0 & $  50\pm11$ \\
13:35:45.47 &  17:47:17.5 & $16.830\pm0.031$ & $0.305\pm0.036$ & $-0.317\pm0.035$ & 1 & $ -26\pm40$ \\
13:35:50.96 &  12:21:18.2 & $18.787\pm0.021$ & $0.939\pm0.037$ & $-0.308\pm0.028$ & 0 & $-109\pm12$ \\
13:36:37.61 &  12:31:42.7 & $15.789\pm0.009$ & $0.977\pm0.025$ & $-0.314\pm0.019$ & 0 & $  17\pm11$ \\
13:38:08.61 &   1:28:05.8 & $15.914\pm0.030$ & $0.605\pm0.034$ & $-0.312\pm0.035$ & 0 & $ 256\pm11$ \\
13:38:15.26 &  -1:59:30.8 & $15.902\pm0.016$ & $0.851\pm0.040$ & $-0.306\pm0.028$ & 0 & $ 219\pm11$ \\
13:43:49.77 &   2:19:32.4 & $16.236\pm0.015$ & $1.046\pm0.029$ & $-0.283\pm0.022$ & 0 & $ 195\pm11$ \\
13:46:41.37 &  20:41:31.9 & $16.261\pm0.024$ & $0.369\pm0.054$ & $-0.317\pm0.041$ & 1 & $ -36\pm28$ \\
13:47:12.75 &  15:21:07.3 & $16.326\pm0.020$ & $0.938\pm0.039$ & $-0.292\pm0.030$ & 0 & $ -14\pm12$ \\
13:49:22.58 &  -0:35:03.3 & $16.937\pm0.021$ & $0.286\pm0.026$ & $-0.345\pm0.025$ & 1 & $  -4\pm40$ \\
13:49:24.51 &  21:07:25.0 & $16.865\pm0.031$ & $0.132\pm0.039$ & $-0.397\pm0.033$ & 1 & $ -47\pm36$ \\
13:49:54.93 &  -0:00:28.3 & $15.892\pm0.025$ & $0.385\pm0.033$ & $-0.343\pm0.029$ & 0 & $ 116\pm12$ \\
13:53:08.80 &   2:56:15.3 & $15.297\pm0.014$ & $0.953\pm0.021$ & $-0.291\pm0.026$ & 0 & $ -28\pm16$ \\
13:53:13.89 &  -3:15:55.5 & $17.719\pm0.027$ & $0.502\pm0.035$ & $-0.340\pm0.030$ & 0 & $ 124\pm11$ \\
13:53:47.55 &  18:30:59.5 & $16.314\pm0.025$ & $0.270\pm0.033$ & $-0.334\pm0.031$ & 1 & $  47\pm30$ \\
13:54:14.51 &   8:34:37.5 & $16.239\pm0.016$ & $0.987\pm0.026$ & $-0.288\pm0.026$ & 0 & $ -62\pm11$ \\
13:56:41.18 &  19:36:46.5 & $16.979\pm0.023$ & $1.178\pm0.114$ & $-0.295\pm0.027$ & 0 & $  40\pm14$ \\
13:57:13.43 &  22:44:33.9 & $16.023\pm0.011$ & $0.356\pm0.025$ & $-0.346\pm0.019$ & 0 & $ -84\pm14$ \\
13:57:29.87 &  20:23:40.6 & $16.234\pm0.027$ & $1.138\pm0.033$ & $-0.293\pm0.041$ & 0 & $ 104\pm12$ \\
13:57:29.89 &   9:23:44.0 & $15.608\pm0.009$ & $0.965\pm0.016$ & $-0.284\pm0.018$ & 0 & $  18\pm11$ \\
13:58:06.58 &  21:12:31.0 & $18.582\pm0.024$ & $0.971\pm0.047$ & $-0.338\pm0.038$ & 0 & $  21\pm11$ \\
14:01:26.10 &  10:02:23.7 & $18.759\pm0.017$ & $0.889\pm0.042$ & $-0.276\pm0.022$ & 0 & $-163\pm16$ \\
14:04:54.23 &  17:51:46.7 & $17.060\pm0.016$ & $0.193\pm0.021$ & $-0.337\pm0.019$ & 1 & $ -27\pm40$ \\
14:14:58.72 &  15:46:22.4 & $16.368\pm0.020$ & $0.417\pm0.025$ & $-0.320\pm0.026$ & 1 & $  42\pm48$ \\
14:18:38.44 &  21:06:11.6 & $17.067\pm0.016$ & $0.187\pm0.024$ & $-0.319\pm0.023$ & 1 & $ -47\pm36$ \\
14:19:05.85 &  18:20:58.3 & $15.141\pm0.051$ & $1.260\pm0.053$ & $-0.330\pm0.065$ & 0 & $  58\pm18$ \\
14:19:19.22 &  -0:40:10.3 & $16.027\pm0.035$ & $1.012\pm0.041$ & $-0.296\pm0.039$ & 0 & $  58\pm14$ \\
14:20:49.02 &  16:13:08.4 & $16.784\pm0.017$ & $0.439\pm0.027$ & $-0.359\pm0.026$ & 0 & $ -92\pm12$ \\
14:21:16.49 &  -3:03:59.3 & $17.896\pm0.023$ & $0.838\pm0.035$ & $-0.304\pm0.027$ & 0 & $-108\pm10$ \\
14:21:31.21 &  -0:44:23.2 & $16.408\pm0.023$ & $0.225\pm0.037$ & $-0.360\pm0.033$ & 1 & $ -61\pm48$ \\
14:24:16.87 &  -1:43:35.0 & $16.384\pm0.015$ & $0.222\pm0.023$ & $-0.349\pm0.023$ & 0 & $ 118\pm15$ \\
14:24:19.66 &  15:07:09.2 & $15.611\pm0.019$ & $1.007\pm0.027$ & $-0.286\pm0.025$ & 0 & $-219\pm11$ \\
14:24:50.97 &  20:21:49.7 & $19.569\pm0.035$ & $1.098\pm0.093$ & $-0.286\pm0.043$ & 0 & $  37\pm15$ \\
14:24:56.10 &   2:13:54.8 & $16.367\pm0.018$ & $1.040\pm0.027$ & $-0.292\pm0.022$ & 0 & $ -53\pm12$ \\
14:25:28.80 &  14:20:59.2 & $16.468\pm0.019$ & $0.119\pm0.026$ & $-0.346\pm0.026$ & 1 & $ 139\pm44$ \\
14:26:32.66 &  18:21:16.2 & $15.641\pm0.019$ & $1.107\pm0.032$ & $-0.312\pm0.028$ & 0 & $  98\pm11$ \\
14:30:05.54 &  20:37:00.1 & $15.749\pm0.019$ & $1.213\pm0.027$ & $-0.281\pm0.026$ & 0 & $ -50\pm11$ \\
14:30:10.73 &   1:33:22.6 & $16.607\pm0.017$ & $0.315\pm0.024$ & $-0.371\pm0.028$ & 0 & $ -18\pm11$ \\
14:30:51.72 &  -2:31:50.8 & $16.699\pm0.020$ & $0.900\pm0.028$ & $-0.281\pm0.026$ & 0 & $ 308\pm19$ \\
14:32:46.80 &   6:21:58.5 & $15.682\pm0.013$ & $0.152\pm0.019$ & $-0.416\pm0.023$ & 0 & $  75\pm13$ \\
14:35:09.40 &   5:46:31.7 & $16.606\pm0.019$ & $0.134\pm0.023$ & $-0.364\pm0.026$ & 1 & $  54\pm28$ \\
14:35:17.27 &  -2:31:27.0 & $17.467\pm0.019$ & $0.974\pm0.029$ & $-0.283\pm0.024$ & 0 & $  32\pm11$ \\
14:35:20.86 &  14:28:40.7 & $16.232\pm0.020$ & $0.190\pm0.028$ & $-0.319\pm0.025$ & 1 & $ 195\pm43$ \\
14:35:50.25 &  18:57:10.7 & $17.304\pm0.018$ & $0.388\pm0.047$ & $-0.345\pm0.025$ & 0 & $-160\pm12$ \\
14:36:20.84 &  -0:06:24.3 & $15.672\pm0.018$ & $0.791\pm0.028$ & $-0.347\pm0.023$ & 0 & $ -88\pm12$ \\
14:36:37.27 &  17:59:42.2 & $16.964\pm0.021$ & $0.496\pm0.028$ & $-0.311\pm0.026$ & 0 & $ -11\pm13$ \\
14:37:23.64 &   6:42:58.4 & $19.613\pm0.026$ & $0.844\pm0.063$ & $-0.358\pm0.036$ & 0 & $  -3\pm21$ \\
14:37:31.84 &  -0:43:28.1 & $15.942\pm0.026$ & $0.942\pm0.033$ & $-0.302\pm0.031$ & 0 & $  75\pm10$ \\
14:38:28.88 &  -2:05:08.7 & $18.062\pm0.024$ & $0.829\pm0.035$ & $-0.274\pm0.029$ & 0 & $ -45\pm10$ \\
14:38:29.12 &  -2:46:50.6 & $15.950\pm0.015$ & $0.910\pm0.024$ & $-0.291\pm0.021$ & 0 & $  -6\pm14$ \\
14:39:39.10 &  11:15:31.4 & $18.438\pm0.019$ & $0.391\pm0.028$ & $-0.343\pm0.031$ & 1 & $ -48\pm21$ \\
14:39:54.90 &   4:52:41.2 & $18.932\pm0.018$ & $0.883\pm0.040$ & $-0.282\pm0.025$ & 0 & $  68\pm13$ \\
14:41:31.66 &  -1:41:23.1 & $17.588\pm0.018$ & $0.929\pm0.028$ & $-0.310\pm0.026$ & 0 & $-136\pm11$ \\
14:42:14.42 &  -0:16:08.2 & $16.333\pm0.015$ & $0.661\pm0.023$ & $-0.284\pm0.025$ & 0 & $ 118\pm13$ \\
14:43:00.26 &  -0:56:50.5 & $18.566\pm0.018$ & $0.825\pm0.033$ & $-0.315\pm0.027$ & 0 & $  97\pm10$ \\
14:43:04.49 &  12:07:12.8 & $18.462\pm0.014$ & $0.870\pm0.031$ & $-0.251\pm0.023$ & 0 & $-109\pm14$ \\
14:44:07.15 &  -0:26:17.7 & $19.329\pm0.020$ & $1.067\pm0.057$ & $-0.301\pm0.027$ & 0 & $  17\pm12$ \\
14:45:04.98 &  14:54:40.2 & $15.808\pm0.018$ & $0.925\pm0.023$ & $-0.317\pm0.025$ & 0 & $  56\pm10$ \\
14:45:08.08 &  10:27:22.6 & $19.168\pm0.016$ & $1.156\pm0.055$ & $-0.289\pm0.024$ & 0 & $-123\pm14$ \\
14:45:13.66 &   1:01:12.8 & $17.096\pm0.022$ & $0.275\pm0.027$ & $-0.396\pm0.030$ & 0 & $  64\pm17$ \\
14:45:33.28 &  16:42:33.4 & $16.399\pm0.021$ & $0.296\pm0.037$ & $-0.355\pm0.024$ & 0 & $ 132\pm13$ \\
14:46:07.42 &   6:58:21.7 & $17.859\pm0.018$ & $0.821\pm0.032$ & $-0.261\pm0.023$ & 0 & $ 124\pm11$ \\
14:47:29.44 &   3:15:05.8 & $16.177\pm0.020$ & $0.129\pm0.030$ & $-0.417\pm0.026$ & 0 & $  98\pm13$ \\
14:48:01.13 &  13:42:32.8 & $19.305\pm0.023$ & $0.581\pm0.047$ & $-0.286\pm0.033$ & 1 & $  50\pm32$ \\
14:48:25.06 &  14:14:51.7 & $19.537\pm0.027$ & $0.501\pm0.055$ & $-0.318\pm0.035$ & 1 & $  75\pm46$ \\
14:49:10.57 &  13:17:09.9 & $16.758\pm0.017$ & $1.056\pm0.025$ & $-0.298\pm0.023$ & 0 & $ -91\pm12$ \\
14:49:24.82 &  16:05:37.1 & $15.562\pm0.018$ & $0.153\pm0.021$ & $-0.384\pm0.022$ & 0 & $  11\pm12$ \\
14:50:40.30 &  20:22:50.3 & $17.510\pm0.018$ & $0.571\pm0.028$ & $-0.302\pm0.022$ & 0 & $  34\pm11$ \\
14:52:23.48 &   5:09:41.2 & $18.217\pm0.016$ & $1.136\pm0.040$ & $-0.285\pm0.023$ & 0 & $ -15\pm12$ \\
14:52:58.42 &  13:27:36.3 & $16.062\pm0.022$ & $0.461\pm0.035$ & $-0.359\pm0.028$ & 0 & $ 114\pm12$ \\
14:54:37.98 &  18:47:25.6 & $16.712\pm0.021$ & $0.149\pm0.033$ & $-0.355\pm0.027$ & 1 & $  98\pm38$ \\
14:54:57.57 &  19:38:54.9 & $16.710\pm0.026$ & $0.947\pm0.030$ & $-0.289\pm0.029$ & 0 & $ 123\pm11$ \\
14:58:10.34 &  18:18:43.4 & $17.955\pm0.017$ & $0.839\pm0.026$ & $-0.278\pm0.023$ & 0 & $ 113\pm14$ \\
14:59:25.52 &  12:52:21.5 & $16.708\pm0.023$ & $0.900\pm0.030$ & $-0.318\pm0.027$ & 0 & $ -52\pm10$ \\
15:01:32.86 &  14:16:04.5 & $16.672\pm0.014$ & $0.859\pm0.021$ & $-0.311\pm0.018$ & 0 & $ -80\pm12$ \\
15:01:50.23 &  13:05:49.2 & $16.253\pm0.016$ & $0.119\pm0.026$ & $-0.371\pm0.023$ & 0 & $ -67\pm12$ \\
15:06:25.90 &  14:20:51.9 & $15.551\pm0.024$ & $0.881\pm0.028$ & $-0.303\pm0.027$ & 0 & $  48\pm13$ \\
15:07:02.96 &  14:34:05.4 & $15.726\pm0.018$ & $0.777\pm0.022$ & $-0.282\pm0.028$ & 0 & $ -84\pm14$ \\
15:10:08.16 &  12:39:50.9 & $17.855\pm0.018$ & $0.580\pm0.028$ & $-0.304\pm0.023$ & 0 & $ 122\pm11$ \\
15:12:03.42 &  12:41:45.0 & $18.792\pm0.018$ & $0.864\pm0.038$ & $-0.287\pm0.025$ & 0 & $ -59\pm10$ \\
15:13:21.24 &  16:30:31.6 & $16.657\pm0.016$ & $0.497\pm0.022$ & $-0.315\pm0.021$ & 0 & $  -9\pm12$ \\
15:16:24.02 &  16:21:17.1 & $17.043\pm0.015$ & $0.960\pm0.022$ & $-0.292\pm0.020$ & 0 & $ -94\pm15$ \\
15:16:32.52 &  19:03:06.4 & $17.258\pm0.017$ & $0.616\pm0.025$ & $-0.340\pm0.024$ & 0 & $  22\pm12$ \\
15:16:55.87 &  11:55:00.3 & $15.862\pm0.018$ & $0.242\pm0.022$ & $-0.391\pm0.028$ & 0 & $ -89\pm13$ \\
15:20:57.22 &  14:41:01.3 & $16.437\pm0.015$ & $0.216\pm0.019$ & $-0.316\pm0.019$ & 1 & $ -93\pm43$ \\
15:21:43.16 &  18:29:35.7 & $19.427\pm0.016$ & $1.021\pm0.063$ & $-0.296\pm0.023$ & 0 & $ -58\pm12$ \\
15:22:20.97 &  25:42:59.9 & $19.224\pm0.018$ & $0.972\pm0.050$ & $-0.276\pm0.027$ & 0 & $ -77\pm12$ \\
15:25:06.63 &  12:56:35.0 & $15.642\pm0.015$ & $0.817\pm0.026$ & $-0.332\pm0.019$ & 0 & $ -92\pm12$ \\
15:26:31.11 &  16:02:13.6 & $15.481\pm0.019$ & $1.005\pm0.024$ & $-0.292\pm0.026$ & 0 & $ -82\pm13$ \\
15:29:10.25 &  13:24:07.3 & $17.525\pm0.021$ & $0.791\pm0.030$ & $-0.284\pm0.030$ & 0 & $  14\pm10$ \\
15:38:08.14 &  12:18:06.5 & $16.659\pm0.016$ & $0.732\pm0.023$ & $-0.304\pm0.020$ & 0 & $-191\pm12$ \\
15:38:29.35 &  17:06:45.0 & $16.997\pm0.017$ & $0.622\pm0.023$ & $-0.307\pm0.023$ & 0 & $ -87\pm13$ \\
15:39:19.04 &  63:12:16.2 & $16.493\pm0.027$ & $1.066\pm0.031$ & $-0.288\pm0.033$ & 0 & $-158\pm16$ \\
15:41:20.91 &  64:16:09.7 & $18.570\pm0.017$ & $0.884\pm0.040$ & $-0.314\pm0.024$ & 0 & $ -10\pm10$ \\
15:43:29.39 &  17:12:38.1 & $15.418\pm0.016$ & $0.262\pm0.022$ & $-0.376\pm0.022$ & 0 & $-148\pm13$ \\
15:45:36.23 &  16:04:16.0 & $16.898\pm0.018$ & $0.172\pm0.025$ & $-0.323\pm0.022$ & 1 & $-104\pm34$ \\
15:45:57.70 &  12:55:32.9 & $16.012\pm0.018$ & $0.899\pm0.025$ & $-0.302\pm0.023$ & 0 & $ -45\pm18$ \\
15:46:13.64 &  11:19:34.4 & $17.687\pm0.012$ & $0.878\pm0.024$ & $-0.287\pm0.016$ & 0 & $  -2\pm11$ \\
15:46:42.65 &  12:49:31.2 & $15.177\pm0.016$ & $0.975\pm0.029$ & $-0.289\pm0.023$ & 0 & $   9\pm11$ \\
15:47:28.22 &  13:28:58.8 & $17.055\pm0.016$ & $0.182\pm0.024$ & $-0.324\pm0.019$ & 1 & $   5\pm36$ \\
15:48:06.47 &  15:54:17.2 & $15.273\pm0.013$ & $0.626\pm0.020$ & $-0.312\pm0.017$ & 0 & $-220\pm10$ \\
15:50:48.03 &  14:16:11.7 & $15.537\pm0.014$ & $0.463\pm0.030$ & $-0.374\pm0.021$ & 0 & $-105\pm10$ \\
15:56:53.76 &  60:24:16.3 & $15.933\pm0.011$ & $0.348\pm0.020$ & $-0.351\pm0.016$ & 0 & $-132\pm10$ \\
15:57:19.31 &  15:39:16.4 & $18.147\pm0.017$ & $0.990\pm0.031$ & $-0.289\pm0.021$ & 0 & $-255\pm11$ \\
16:07:11.93 &  17:46:03.5 & $17.821\pm0.013$ & $0.987\pm0.031$ & $-0.279\pm0.018$ & 0 & $ 136\pm10$ \\
16:14:23.42 &  53:14:05.0 & $16.961\pm0.039$ & $0.174\pm0.045$ & $-0.401\pm0.045$ & 0 & $-144\pm12$ \\
16:21:39.65 &  56:09:06.7 & $16.578\pm0.015$ & $0.915\pm0.027$ & $-0.314\pm0.019$ & 0 & $ -83\pm11$ \\
16:23:59.61 &  37:54:35.3 & $15.373\pm0.017$ & $0.459\pm0.023$ & $-0.359\pm0.022$ & 0 & $-248\pm10$ \\
16:24:43.78 &  33:38:25.2 & $16.512\pm0.021$ & $0.282\pm0.030$ & $-0.307\pm0.024$ & 1 & $ -91\pm43$ \\
16:32:31.66 &  54:29:39.6 & $16.707\pm0.012$ & $0.430\pm0.017$ & $-0.359\pm0.022$ & 0 & $ -68\pm11$ \\
16:36:01.24 &  52:50:20.5 & $16.811\pm0.019$ & $0.908\pm0.027$ & $-0.312\pm0.021$ & 0 & $-243\pm11$ \\
16:38:59.57 &  55:37:45.7 & $19.177\pm0.018$ & $0.709\pm0.052$ & $-0.307\pm0.028$ & 0 & $-322\pm11$ \\
16:42:59.22 &  36:23:36.4 & $15.894\pm0.013$ & $0.576\pm0.021$ & $-0.345\pm0.024$ & 0 & $-236\pm11$ \\
16:43:22.72 &  34:34:31.5 & $16.209\pm0.017$ & $1.116\pm0.023$ & $-0.291\pm0.023$ & 0 & $-273\pm11$ \\
16:47:10.83 &  42:23:54.3 & $15.489\pm0.022$ & $0.138\pm0.027$ & $-0.390\pm0.037$ & 0 & $-193\pm10$ \\
16:48:35.99 &  50:30:38.1 & $18.157\pm0.019$ & $0.643\pm0.031$ & $-0.296\pm0.024$ & 0 & $-129\pm10$ \\
16:53:08.88 &  50:25:09.9 & $18.489\pm0.019$ & $0.858\pm0.037$ & $-0.307\pm0.022$ & 0 & $-121\pm11$ \\
16:53:29.02 &  49:37:32.6 & $19.183\pm0.015$ & $0.929\pm0.052$ & $-0.311\pm0.023$ & 0 & $  -3\pm10$ \\
16:53:45.98 &  47:42:28.3 & $17.115\pm0.013$ & $0.597\pm0.025$ & $-0.361\pm0.017$ & 0 & $ -47\pm10$ \\
17:07:38.35 &  43:40:32.9 & $18.693\pm0.017$ & $0.854\pm0.035$ & $-0.289\pm0.022$ & 0 & $-107\pm11$ \\
17:08:11.80 &  43:28:15.4 & $18.464\pm0.018$ & $0.716\pm0.032$ & $-0.305\pm0.027$ & 0 & $-184\pm12$ \\
21:50:28.10 &  -0:30:18.6 & $18.902\pm0.019$ & $0.550\pm0.043$ & $-0.294\pm0.028$ & 0 & $-185\pm11$ \\
22:28:20.78 &  13:11:25.6 & $16.017\pm0.013$ & $0.740\pm0.020$ & $-0.307\pm0.016$ & 0 & $-133\pm11$ \\
22:30:08.25 &  13:27:34.2 & $16.716\pm0.015$ & $0.354\pm0.021$ & $-0.383\pm0.021$ & 0 & $  20\pm14$ \\
22:33:14.90 &  12:19:34.1 & $15.819\pm0.021$ & $0.234\pm0.031$ & $-0.352\pm0.023$ & 0 & $ -17\pm11$ \\
22:39:06.10 &  12:30:34.5 & $16.085\pm0.020$ & $0.191\pm0.026$ & $-0.362\pm0.023$ & 0 & $ -72\pm12$ \\
22:42:31.14 &  12:50:04.9 & $16.223\pm0.018$ & $0.197\pm0.022$ & $-0.328\pm0.022$ & 1 & $  65\pm26$ \\
22:42:46.75 &  14:54:17.8 & $17.181\pm0.016$ & $0.108\pm0.023$ & $-0.364\pm0.021$ & 1 & $  70\pm29$ \\
23:01:55.17 &  14:36:00.9 & $15.918\pm0.013$ & $0.227\pm0.019$ & $-0.310\pm0.021$ & 1 & $  19\pm20$ \\
23:58:51.31 &  15:35:41.0 & $17.061\pm0.016$ & $0.186\pm0.022$ & $-0.346\pm0.021$ & 1 & $ -22\pm28$ \\

